Probing the early Milky Way with GHOST spectra of an extremely metal-poor star in the Galactic disk

Pristine_183.6849+04.8619 (P1836849) is an extremely metal-poor ([Fe/H]$=-3.3\pm0.1$) star on a prograde orbit confined to the Galactic disk. Such stars are rare and may have their origins in protogalactic fragments that formed the early Milky Way, in low mass satellites accreted later, or forming in situ in the Galactic plane. Here we present a chemo-dynamical analysis of the spectral features between $3700-11000$\r{A} from a high-resolution spectrum taken during Science Verification of the new Gemini High-resolution Optical SpecTrograph (GHOST). Spectral features for many chemical elements are analysed (Mg, Al, Si, Ca, Sc, Ti, Cr, Mn, Fe, Ni), and valuable upper limits are determined for others (C, Na, Sr, Ba). This main sequence star exhibits several rare chemical signatures, including (i) extremely low metallicity for a star in the Galactic disk, (ii) very low abundances of the light $\alpha$-elements (Na, Mg, Si) compared to other metal-poor stars, and (iii) unusually large abundances of Cr and Mn, where [Cr, Mn/Fe]$_{\rm NLTE}>+0.5$. A comparison to theoretical yields from supernova models suggests that two low mass Population III objects (one 10 M$_\odot$ supernova and one 17 M$_\odot$ hypernova) can reproduce the abundance pattern well (reduced $\chi^2<1$). When this star is compared to other extremely metal-poor stars on quasi-circular, prograde planar orbits, differences in both chemistry and kinematics imply there is little evidence for a common origin. The unique chemistry of P1836849 is discussed in terms of the earliest stages in the formation of the Milky Way.

==> gaia_edr3_table.tex <==
\begin{table*}
\caption{The Pristine names, Gaia DR3 source ID, G, BP-RP, and parallax, and reddening from the 3D map of \citet{Green19}. }
\label{tab:target}
% \resizebox{\textwidth}{!}
\begin{tabular}{cccccccccc}
\hline
Pristine name & Short name & source ID   & G & BP-RP & A$_{\rm V}$ &  $\pi$" & $\sigma$($\pi$") \\
& & & (mag) & (mag) &  (mag)  &  & \\
\hline
Pristine\_183.6849+04.8619   & P1836849 & 3894267325687326592 & 14.82  & 0.62 & 0.05  & 
0.80555 & 0.03386 \\
\hline
\end{tabular}
\end{table*}
